Large-scale visual SLAM for in-the-wild videos

Accurate and robust 3D scene reconstruction from casual, in-the-wild videos can significantly simplify robot deployment to new environments. However, reliable camera pose estimation and scene reconstruction from such unconstrained videos remains an open challenge. Existing visual-only SLAM methods perform well on benchmark datasets but struggle with real-world footage which often exhibits uncontrolled motion including rapid rotations and pure forward movements, textureless regions, and dynamic objects. We analyze the limitations of current methods and introduce a robust pipeline designed to improve 3D reconstruction from casual videos. We build upon recent deep visual odometry methods but increase robustness in several ways. Camera intrinsics are automatically recovered from the first few frames using structure-from-motion. Dynamic objects and less-constrained areas are masked with a predictive model. Additionally, we leverage monocular depth estimates to regularize bundle adjustment, mitigating errors in low-parallax situations. Finally, we integrate place recognition and loop closure to reduce long-term drift and refine both intrinsics and pose estimates through global bundle adjustment. We demonstrate large-scale contiguous 3D models from several online videos in various environments. In contrast, baseline methods typically produce locally inconsistent results at several points, producing separate segments or distorted maps. In lieu of ground-truth pose data, we evaluate map consistency, execution time and visual accuracy of re-rendered NeRF models. Our proposed system establishes a new baseline for visual reconstruction from casual uncontrolled videos found online, demonstrating more consistent reconstructions over longer sequences of in-the-wild videos than previously achieved.

==> introduction-v1.tex <==

% our motivation and contributions
% There are many videos on the Internet; these videos can be a great source for the training of generative AI if we can successfully reconstruct these videos.
In the SLAM community, benchmark datasets are typically collected using sensors mounted on robots navigating controlled or uncontrolled environments.
These sensor readings are then processed and shared with the community making creating new datasets a resource intensive activity.
On the other hand, numerous freely available online videos, such as city tours and egocentric recordings, offer similar yet more challenging and realistic data.
Therefore, we propose investigating the feasibility of leveraging these video sources to develop and evaluate SLAM algorithms.


% The motivation
However, the accurate reconstruction of 3D scenes and estimation of camera poses from in-the-wild videos---such as city tours or egocentric recordings---continues to be a critical challenge for simultaneous localization and mapping.
Although previous visual reconstruction methods have demonstrated significant success on benchmark datasets~\cite{geiger2013vision,sturm2012benchmark,straub2019replica}, they frequently encounter difficulties when applied to public videos found online, particularly in the case of large camera rotations, lack of distinctive features, and dynamic scenes.
Given recent advancements in drone control~\cite{reference} and the increasing agility of mobile robots---such as those developed by Boston Dynamics---the prevalence of such challenging visual inputs is bound to grow.
% Previous visual reconstruction methods have demonstrated significant success on established datasets~\cite{geiger2013vision,sturm2012benchmark,straub2019replica}. However, estimating camera motion and reconstructing scene geometry from in-the-wild videos (such as egocentric recordings or city-tour footage from YouTube) remains a challenging problem.

% Why it is difficult and examples
More specifically---as we will show in our experiments and analysis section (\cref{section_label})---current visual SLAM~\cite{mur2015orb} and SfM~\cite{schonberger2016structure} methods often fail and generate multiple separate trajectories due to: 1) small-parallax motion during the recording and; 2) insufficient reliable correspondence estimations across frames.
First, for those in-the-wild videos (like city walking tour videos), it is very common for the camera movement to be dominated by pure rotation and forward.
% Is it clear?
Pure rotations can result in low overlap between frames, and more importantly, the small baselines between cameras will result in high uncertainty of depth estimation.
Second, due to the dynamic objects and texture-poor regions in the view, the estimated correspondence between frames are not reliable, resulting in incorrect pose estimation or complete failure.
% Third, those in-the-wild videos often consist of thousands of frames,



In this work, we aim to do visual reconstruction on in-the-wild videos, especially those recorded city-walking tour recordings.
During the reconstruction, we care more about robustness than accuracy;
that is to say, we want to generate one consistent trajectory.
Given the failure analysis above, we try to fix them and build our reconstruction pipeline upon the visual SLAM system \textit{DPVO}~\cite{teed2024deep}.
% our contributions (what we did)
We choose \textit{DPVO} as our basis because of its efficiency and reliability of correspondence estimation.
Instead of key-point detection and feature matching, DPVO estimates frame-to-frame correspondence by evaluating the deep optical flow, which can handle texture-poor regions well.
Our goal is a complete system that can run on random videos.
To achieve this, we start from a global SfM reconstruction on the first few frames to estimate coarse initial camera intrinsics.
With this initial estimate of the intrinsics, we run the visual SLAM in a sliding window way by evaluating the optical flow difference.
To handle the depth ambiguity due to the small baselines, we adopt  off-the-shelf monocular depth estimation as prior information and regularization to guide  bundle adjustment.
To handle dynamic objects in the view, we use semantic detection to generate dynamic masks, and also, avoid sampling on those less-constraint regions such as the sky.
Our experiments show that the proposed depth regularization term can help reduce the depth ambiguity and maintain the scene scale effectively.
In the visual SLAM process, pose drift is often unavoidable. To reduce the drift during the reconstruction, we add loop closure optimization on $\texttt{SIM(3)}$~\cite{strasdat2010scale} to reduce the estimation drift.
As a post-processing step, we run a global bundle adjustment to refine the camera's intrinsic parameters and poses in one pass.

